Text-guided Synthetic Geometric Augmentation for Zero-shot 3D Understanding

Zero-shot recognition models require extensive training data for generalization. However, in zero-shot 3D classification, collecting 3D data and captions is costly and laborintensive, posing a significant barrier compared to 2D vision. Recent advances in generative models have achieved unprecedented realism in synthetic data production, and recent research shows the potential for using generated data as training data. Here, naturally raising the question: Can synthetic 3D data generated by generative models be used as expanding limited 3D datasets? In response, we present a synthetic 3D dataset expansion method, Textguided Geometric Augmentation (TeGA). TeGA is tailored for language-image-3D pretraining, which achieves SoTA in zero-shot 3D classification, and uses a generative textto-3D model to enhance and extend limited 3D datasets. Specifically, we automatically generate text-guided synthetic 3D data and introduce a consistency filtering strategy to discard noisy samples where semantics and geometric shapes do not match with text. In the experiment to double the original dataset size using TeGA, our approach demonstrates improvements over the baselines, achieving zeroshot performance gains of 3.0% on Objaverse-LVIS, 4.6% on ScanObjectNN, and 8.7% on ModelNet40. These results demonstrate that TeGA effectively bridges the 3D data gap, enabling robust zero-shot 3D classification even with limited real training data and paving the way for zero-shot 3D vision application.

==> tables/exploratory_experiments.tex <==
\begin{table*}[t]
\begin{tabular}{ccc}

\begin{minipage}[t]{0.32\hsize}
\begin{center}
 \caption{Effect of pormpt augmentation.}
 \vspace{-10pt}
 \scalebox{0.87}{
 \begin{tabular}{l|cccc} 
 \toprule[0.8pt]
    \multirow{2}*{Prompt type} & O-LVIS & S-Object & M40 \\
    & Top1 & Top1 & Top1 \\
 \midrule[0.5pt]
     Category & -- & -- & -- \\
     Caption & -- & -- & -- \\
 \bottomrule[0.8pt]
  \end{tabular}
\label{tab:prompt_augmentation}
 }
\end{center}
\end{minipage}
 \begin{minipage}[t]{0.36\hsize}
\caption{Effect of consistency filtering.} 
 \vspace{-19pt}
 \begin{center}
\scalebox{0.87}{
 \begin{tabular}{l|cccc} 
 \toprule[0.8pt]
    \multirow{2}*{Filtering} & O-LVIS & S-Object & M40 \\
    & Top1 & Top1 & Top1 \\
 \midrule[0.5pt]
      w/o filtering  & -- & -- & -- \\
     w/ filtering & -- & -- & -- \\
 \bottomrule[0.8pt]
 \end{tabular}
\label{tab:data_representation}
   }
\end{center}
  \end{minipage}

\begin{minipage}[t]{0.29\hsize}
  \caption{Effect of guidance scale.}
   \vspace{-20pt}
\begin{center}
\scalebox{0.87}{
 \begin{tabular}{l|cccc} 
 \toprule[0.8pt]
    \multirow{2}*{Value} & O-LVIS & S-Object & M40 \\
    & Top1 & Top1 & Top1 \\
 \midrule[0.5pt]
     0.3  & -- & -- & -- \\
     3.0 & -- & -- & -- \\
     30 & -- & -- & -- \\
 \bottomrule[0.8pt]
 \end{tabular}
\label{tab:effect_of_loss}
  }
\end{center}
  \end{minipage}
     \end{tabular}

\vspace{-10pt}
\end{table*}


==> tables/tab_con_vs_scon.tex <==
% \begin{table}[t]
%   \centering
%   \setlength{\tabcolsep}{7pt}
%   \caption{Ablation studies of the design of fusion function $g^{MV}$. 
%   We report results on Objaverse-LVIS (O-LVIS) and ScanObjectNN (S-Object).}  \resizebox{0.98\linewidth}{!}{
%   \begin{tabular}{l|cccccccc}
%     \toprule
%     \multirow{2}*{Scaling} & M40 & O-LVIS & S-Object \\
%     & Top1 & Top1 & Top1\\
%     \midrule
%     Contrastive & -- & -- & -- \\
%     Supervised Contrastive  & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:real_synthetic_ratio}
% \end{table}

==> tables/tab_pointe_vs_fractals.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{7pt}
  \caption{Ablation studies of synthetic geometric representation.}  
  \vspace{-10pt}
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{c|cccccccc}
    \toprule
    \multirow{2}*{Dataset} & O-LVIS & S-Object & M40 \\
    & Top1 & Top1 & Top1\\
    \midrule
    Semantics shape  & 11.5 & 46.6 & 71.1 \\
    Fractal shape & -- & -- & -- \\
    \bottomrule
  \end{tabular}}
  \label{tab:semantics_vs_fractal}
  % \vspace{12pt}
\end{table}

==> tables/tab_prompt_augmentation.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{7pt}
  \caption{Effect of prompt augmentation. 
  We report results on ModelNet40 (M40), Objaverse-LVIS (O-LVIS) and ScanObjectNN (S-Object).}  
  \vspace{-10pt}
  \resizebox{0.98\linewidth}{!}{
  \begin{tabular}{l|cccccccc}
    \toprule
    \multirow{2}*{Prompt} & M40 & O-LVIS & S-Object \\
    & Top1 & Top1 & Top1\\
    \midrule
    category & -- & -- & -- \\
    GPT-4 caption & -- & -- & -- \\
    % category + ** & -- & -- & -- \\
    \bottomrule
  \end{tabular}}
  \label{tab:prompt_augmentation}
\end{table}

==> tables/tab_testdata_augmentation.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{7pt}
  \caption{Ablation studies of the design of fusion function $g^{MV}$. 
  We report results on Objaverse-LVIS (O-LVIS) and ScanObjectNN (S-Object).}  \resizebox{0.98\linewidth}{!}{
  \begin{tabular}{l|cccccccc}
    \toprule
    \multirow{2}*{Prompt} & O-LVIS & M40 & S-Object \\
    & Top1 & Top1 & Top1\\
    \midrule
    ShapeNet & -- & -- & -- \\
    + O-LVIS + S-Object + M40 & -- & -- & -- \\
    \bottomrule
  \end{tabular}}
  \label{tab:real_synthetic_ratio}
\end{table}
